Beating the thermal limit of qubit initialization with a Bayesian Maxwell's demon

Fault-tolerant quantum computing requires initializing the quantum register in a well-defined fiducial state. In solid-state systems, this is typically achieved through thermalization to a cold reservoir, such that the initialization fidelity is fundamentally limited by temperature. Here, we present a method of preparing a fiducial quantum state with a confidence beyond the thermal limit. It is based on real time monitoring of the qubit through a negative-result measurement -- the equivalent of a `Maxwell's demon' that triggers the experiment only upon the appearance of a qubit in the lowest-energy state. We experimentally apply it to initialize an electron spin qubit in silicon, achieving a ground-state initialization fidelity of 98.9(4)%, corresponding to a 20$\times$ reduction in initialization error compared to the unmonitored system. A fidelity approaching 99.9% could be achieved with realistic improvements in the bandwidth of the amplifier chain or by slowing down the rate of electron tunneling from the reservoir. We use a nuclear spin ancilla, measured in quantum nondemolition mode, to prove the value of the electron initialization fidelity far beyond the intrinsic fidelity of the electron readout. However, the method itself does not require an ancilla for its execution, saving the need for additional resources. The quantitative analysis of the initialization fidelity reveals that a simple picture of spin-dependent electron tunneling does not correctly describe the data. Our digital `Maxwell's demon' can be applied to a wide range of quantum systems, with minimal demands on control and detection hardware.

==> Bayesian Maxwell's demon manuscript/glossary.tex <==
\newacronym{set}{SET}{single electron transistor}
\newacronym{nmr}{NMR}{nuclear magnetic resonance}
\newacronym{esr}{ESR}{electron spin resonance}
\newacronym{spam}{SPAM}{state preparation and measurement}
\newacronym{qnd}{QND}{quantum nondemolition}
\newacronym{fpga}{FPGA}{field-progammable gate array}
\newacronym{qpc}{QPC}{quantum point contact}
\newacronym{cp}{CP}{Carr-Purcell}
\newacronym{cpmg}{CPMG}{Carr-Purcell-Meiboom-Gill}

==> Bayesian Maxwell's demon manuscript/preamble.tex <==
% Revtex stuff
\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{bm}% bold math
\usepackage{hyperref}% add hypertext capabilities
% \usepackage[mathlines]{lineno}% Enable numbering of text and display math
% \linenumbers\relax % Commence numbering lines

\usepackage[utf8]{inputenc}

\usepackage{graphicx}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{lipsum}
\usepackage{glossaries}

\usepackage{siunitx}
\usepackage{braket}


\usepackage{mathtools}
\DeclarePairedDelimiter{\Tr}{\textnormal{Tr}[}{]}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}%
\DeclarePairedDelimiter\expectation{\langle}{\rangle}%

\newcommand{\prob}[1]{\ensuremath{P(#1)}}
\newcommand{\pgiv}[2]{\ensuremath{P(#1 \,\mid #2)}}
\newcommand{\likelihood}[2]{\ensuremath{\mathcal{L}(#1\mid #2)}}



%Required by revtex
\usepackage{natbib}
% \usepackage{subcaption}
% \usepack%age{pdfpages}

% \usepackage[subpreambles=true]{standalone}
% \usepackage{import}

\usepackage{xcolor}
% For comments
\newcommand{\com}[1]{$\clubsuit$ {\color{blue}#1} $\clubsuit$}

\definecolor{commentgreen}{RGB}{2,112,10}
\definecolor{eminence}{RGB}{108,48,130}
\definecolor{weborange}{RGB}{255,165,0}
\definecolor{frenchplum}{RGB}{129,20,83}
\usepackage{listings}
\lstset {
    language=Verilog,
    frame=tb,
    tabsize=4,
    showstringspaces=false,
    numbers=left,
    %upquote=true,
    commentstyle=\color{commentgreen},
    keywordstyle=\color{eminence},
    stringstyle=\color{red},
    basicstyle=\small\ttfamily, % basic font setting
    emphstyle={\color{blue}},
    escapechar=\&,
    % keyword highlighting
    classoffset=1, % starting new class
%    otherkeywords={>,<,.,;,-,!,=,~},
%    morekeywords={>,<,.,;,-,!,=,~},
    keywordstyle=\color{weborange},
    classoffset=0,
}
